Swapping: a natural bridge between named and indexed explicit substitution calculi

This article is devoted to the presentation of lambda_rex, an explicit substitution calculus with de Bruijn indexes and a simple notation. By being isomorphic to lambda_ex - a recent formalism with variable names -, lambda_rex accomplishes simulation of beta-reduction (Sim), preservation of beta-strong normalization (PSN) and meta-confluence (MC), among other desirable properties. Our calculus is based on a novel presentation of lambda_dB, using a swap notion that was originally devised by de Bruijn. Besides lambda_rex, two other indexed calculi isomorphic to lambda_x and lambda_xgc are presented, demonstrating the potential of our technique when applied to the design of indexed versions of known named calculi.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{E. Bonelli (Ed.): 5th International Workshop\\
on Higher-Order Rewriting (HOR'10)\\
EPTCS 49, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.49.1}{10.4204/EPTCS.49.1}}
\pdfoutput=1

